FLARE: Fault Attack Leveraging Address Reconfiguration Exploits in Multi-Tenant FPGAs

Modern FPGAs are increasingly supporting multi-tenancy to enable dynamic reconfiguration of user modules. While multi-tenant FPGAs improve utilization and flexibility, this paradigm introduces critical security threats. In this paper, we present FLARE, a fault attack that exploits vulnerabilities in the partial reconfiguration process, specifically while a user bitstream is being uploaded to the FPGA by a reconfiguration manager. Unlike traditional fault attacks that operate during module runtime, FLARE injects faults in the bitstream during its reconfiguration, altering the configuration address and redirecting it to unintended partial reconfigurable regions (PRRs). This enables the overwriting of pre-configured co-tenant modules, disrupting their functionality. FLARE leverages power-wasters that activate briefly during the reconfiguration process, making the attack stealthy and more challenging to detect with existing countermeasures. Experimental results on a Xilinx Pynq FPGA demonstrate the effectiveness of FLARE in compromising multiple user bitstreams during the reconfiguration process.

==> add.tex <==
1. structure of bitstream (preemptive reconfiguration, loopbreaker)

2. How much time required during address 'select'?

3. remove ILA from design (so more adders can be accommodated)

70 cycles for the header and next 150 cycles for loading the address



adder# 474 error when 1000 adders are used

when we run 50 times, 37 times adders are getting impacted: attack success =74\%.

100 attempts, 75 faults: attack success=75\%.

200 attempts, 150 faults: attack success=75\%

300, 223 faults, attack success=74.3\%

500, 372 faults, attack success=74.4\%


 Fine-granularity of attacks.

Histogram: (10000)
500 adders: 10 bins, each bin getting attacked. two separate plots for two adder clusters.


Plot:
****
How many times encoder 1 failed?
encoder 2 failed?
adder cluster 1 error?
adder cluster 2 error?

plot with 4 bars 
y-axis: no of times there was an error.
****


add another aes in CoRQ to increase utilization.



 

==> results_to_add.tex <==
case 1: AES

LUTs configured: 38719

No. of times Encoder 1 failed 5100

No. of times Encoder 2 failed 5090

No. of times Adder cluster 1 failed 4885

No. of times Adder cluster 2 failed 4895
